Unraveling the Formation History of the Black Hole X-ray Binary LMC X-3 from ZAMS to Present

We have endeavoured to understand the formation and evolution of the black hole (BH) X-ray binary LMC X-3. We estimate the properties of the system at 4 evolutionary stages: 1) at the Zero Age Main Sequence (ZAMS), 2) just prior to the supernova (SN) explosion of the primary, 3) just after the SN, and 4) at the moment of RLO onset.We use a hybrid approach, combining detailed stellar structure and binary evolution calculations with approximate population synthesis models. This allows us to estimate potential natal kicks and the evolution of the BH spin. In the whole analysis we incorporate as model constraints the most up-to-date observational information, encompassing the binary's orbital properties, the companion star mass, effective temperature, surface gravity and radius, as well as the black hole's mass and spin. We find that LMC X-3 began as a ZAMS system with the mass of the primary star in the range $M_{\rm{1,ZAMS}}$ = 22-31 $\rm{M_{\odot}}$ and a secondary star of $M_{\rm{2,ZAMS}} = 5.0-8.3M_{\odot}$, in a wide ($P_{ZAMS} \gtrsim 2.000\, \rm days$) and eccentric ($e_{\rm{ZAMS}} \gtrsim 0.23$) orbit. Just prior to the SN, the primary has a mass of $M_{\mathrm{1,preSN}} = 11.1-18.0\,\rm M_{\odot}$, with the secondary star largely unaffected. The orbital period decreases to $0.6-1.7\, \rm days$, and is still eccentric $0 \leq e_{\rm{preSN}} \leq 0.44$. We find that a symmetric SN explosion with no or small natal kicks (a few tens of $\rm km\, s^{-1}$) imparted on the BH cannot be formally excluded, however, large natal kicks in excess of $\gtrsim 120 \,\rm km\, s^{-1}$ increase the estimated formation rate by an order of magnitude. Following the SN, the system has a BH $M_{\mathrm{BH,postSN}} = 6.4-8.2\,\rm M_{\odot}$ and is put into an eccentric orbit. At the RLO onset the orbit is circularised and it has an orbital period of $P_{\rm{RLO}} = 0.8-1.4\,\rm days$.

==> b_kick.tex <==
%\section{Coordinate system and Velocity components}
%With right ascension $alpha_0$, declination $\delta_0$, and distance $D_0$ we define on the celestial sphere $\mathcal{O} = (\alpha_0, 
%\delta_0, D_0)$ as the origin for the LMC center of mass and introduce on to this a cartisian coordinate system (x,y,z). Here the x-axis is %positive in the antiparallel direction of $\alpha_0$, the y-axis is parallel to the declinaiton axis and the z-axis is positive toward the observer.
%Any star being a member of the LMC has right ascension $\alpha$, declination $\delta$, and distance D. In the (x,y,z) coordinate system the %we define $\rho$ 
\section{Supernova induced kick}
When $M_{1}$ went supernova a kick was imparted to the binary system due to an assymmetric explosion. Though the consequence of the kick was not disrupting the system it may have affected the orbit of the binary system within the LMC.
Presumably the binary system center of mass, orbits its parent galaxy like the average field star does with some velocity dispersion. The pre SN velocity then is
\begin{equation}
\vec{v_{pre SN}'} = \vec{v_{rot}'} + \vec{v_{\sigma}'}
\end{equation}
With the SN, the kick is imparted and contributes to the velocity of the binary system center of mass
\begin{equation}
\vec{v_{post SN}'} = \vec{v_{pre SN}'} + \vec{v_{kick}'}
\end{equation}
and the trajectory of the binary system is on a new cours. From BSE the binary system center of mass velocity amplitude 
\begin{equation}
|\vec{v_{kick}'}| = \sqrt{v_{kick,x'}^2 + v_{kick,y'}^2 + v_{kick,z'}^2}
\label{eq:vkickmark}
\end{equation}
is known but the individual components $\vec{v_{kick}} = v_{kick,x'} + v_{kick,y'} + v_{kick,z'}$ are unknown. From \cite{vandermarel2002} we can transform from the coordinate system (x', y',z') into the (x,y,z) system from which we can get the line of sight velocity as measured by an observer.
Eq. 24 of \cite{vandermarel2002} expresses the line of sight velocity for a tracer star in LMC accounting for the center of mass motion of LMC $\vec{v_{LMC CM}}$, the precession and nutation $\vec{v_{pn}}$ due to tidal torques from external forces, and the internal rotation of the tracer stars, $\vec{v_{int}}$. If the LMC X-3 experienced a kick when going SN, this introduces a fourth component which is $\vec{v_{kick}'}$ given in eq. \eqref{eq:vkickmark}.

==> layout.tex <==
*** Introduction

Start with a few of paragraphs that are at low level, wikipedia style, where you introduce: 
1) what X-ray binaries are, 2) what is the standard formation channel that we consider, 
3) why is it useful to try to reconstruct the evolutionary history of BH XRBs, 
4) summarize the work that has being done so far (earlier papers from the same project, my LMXB spin paper, the recent paper on M82 X-2 (http://adsabs.harvard.edu/abs/2015arXiv150102679F) Repetto, S., Davies, M. B., & Sigurdsson, S. (2012)., other similar work)
5) Try to make a point of why LMC X-3 is especially interesting: different metallicity, good distant measurement which results precise and robust measurements. Rare class of intermediate-mass X-ray binaries.

6) Mention very briefly in one paragraph what is the goal and methodology of the paper.
7) End with a paragraph where you mention what is in each of the next sections.

*** Observational Constrains

1) You can start with a historical review of of LMC X-3 discovery and first observations
2) A table with all the observational constraints we are going to use. In the text that refers to the table mention explicitly that we are considering 2-sigma errors.
3) You can also mention any other interesting observational properties.  

*** Star formation history in the neighborhood of LMC X-3
This section will be probably written by Valia, and will include the photometric observations we were looking at in the first skype meetings

*** Methodology
Here you could have a longer description of the methodology with the sketch that you will make.


*** MT calculations
Here you could have 4 subsections:
-- The description of the code and the setup you use, along the choice of parameters. 
-- A description of the finite part of the parameter space that we have to cover. The initial scan of the parameter space with the fiducial MT calculation.
-- Describe how you search for winners, and show a few different indicative MT sequences describing qualitative how the MT sequences behave in different part of the parameter space.
-- Present a summary of all the winning MT sequences and have one summary table of the derived constraints at the onset of RLO, and a full table with all the winning sequences one by one. Only a part of the table will be in the actual table and the full version will be only online

*** Supernova dynamics and post-SN detached orbital evolution
this part will of course have to wait, but you will first have to describe in detail the equation you will use for both the dynamics and the tidal evolution, and then present the pre-SN constraints you derive

*** Population synthesis simulations with BSE (we will talk more about this code)
In this part you will do the approximate evolution of binaries from birth until right before the SN (including the common envelope). This part will also take into account the distributions of initial binary properties of a general binary population. That way, we will not only know which pre-SN configuration are possible, but also which ones are the most probable.

*** Final Probability density distributions
Here we will combine the the population synthesis calculation with the constraints from the previous steps and derive probability density distributions for each property of LMC X-3, at different stages of its evolution

*** Summary and conclusions
Here you can start with one or two paragraphs of what we do in this paper
Then you should enumerate our main findings and conclusions
